Some aspects of quantum correlations and decoherence in the cosmological spacetimes

This thesis presents a theoretical investigation into the quantum field theoretic aspects of quantum correlations and decoherence in the cosmological spacetimes. We shall focus on the inflationary or dark energy dominated phase of the universe, and we shall take the spacetime background to be de Sitter. The primary objective of this thesis is to study the physics of the very early universe and to gain insight into the interesting interplay among quantum correlations, entanglement and decoherence which can affect the evolution of our universe.

==> plist.tex <==
\centerline{\bf \Large List of Publications}
\vskip .5in
\thispagestyle{empty}
{\bf Peer-reviewed Journals:}
\vskip .4in
\makeatletter
\renewcommand{\theenumi}{\arabic{enumi}}
%\renewcommand{\labelenumi}{\theenumi.}
\makeatother
\begin{enumerate}

\item \textbf{Shagun Kaushal} and S. Sarkar, “Dependence of the far-field optical response of ion beam sculpted Cu thin films on their surface'', \textbf{Appl. Surf. Sci.}, {526}, 146473 (2020).
\url{https://doi.org/10.1016/j.apsusc.2020.146473}
\item \textbf{Shinki} and S. Sarkar, “Au$_{0.5}$ Ag $_{0.5}$ Alloy Nanolayer Deposited on Pyramidal Si Arrays as Substrates for Surface-Enhanced Raman Spectroscopy”, \textbf{ACS Appl. Nano Mater.} {3}, 7088-7095 (2020).\url{https://doi.org/10.1021/acsanm.0c01407}
\item \textbf{Shinki}, J.Singh and S. Sarkar, “Tuning the topographical parameters of Si pyramids for a better surface enhanced Raman response”, \textbf{Phys. Chem. Chem. Phys.} {23}, 26407-26416 (2021).\url{	https://doi.org/10.1039/D1CP03576B}
\item \textbf{Shinki}, S.Jain and S. Sarkar, “Role of Au–Ag alloy plasmonic layer thickness over pyramidal silicon in controlling SERS activity”, \textbf{Eur. Phys. J. Spec. Top.} {},  231, 791–797 (2022).\url{ https://doi.org/10.1140/epjs/s11734-022-00463-3}
\item \textbf{Shinki} and S. Sarkar, “Day life candidate as flexible substrates for pesticide detection : A
comparative study” \textbf{Plasmonics}, 17, 1293-1303 (2022).
\url{ https://doi.org/10.1007/s11468-022-01618-7}
\item \textbf{Shinki} and S. Sarkar, “Is 3D surface structuring always a prerequisite for effective SERS ?”  \textbf{Surfaces and Interfaces}, 33, 102223 (2022).
\url{https://doi.org/10.1016/j.surfin.2022.102223}
\end{enumerate}
%\hspace{0.2in}
\vskip .7in
{\bf Conference Paper:}
\begin{enumerate}
\item 
Aditi Chopra, Megha Lekhi, \textbf{Shinki}, Subhendu Sarkar and Sudipta Sarkar Pal ``Investigation of plasmonic nanostructures with controlled roughness as SERS substrate'', Page No. TP138 \textbf{(Photonics 2018)}
\end{enumerate}
\vskip .4in
{\bf Book Chapter:}
\begin{enumerate}
\item 
Shinki and Subhendu Sarkar, ``Perspectives and Fabrication Challenges for Plasmon-Based SERS Substrates'' in  \textit{\textbf{Encyclopedia of Materials: Electronics}}, Elsevier (2023).
\end{enumerate}

==> presentations.tex <==
\centerline{\bf \Large Presentations and Conferences}
\thispagestyle{empty}
\vskip .5in



{\bf Poster Presentation:}

\makeatletter
\renewcommand{\theenumi}{\arabic{enumi}}
%\renewcommand{\labelenumi}{\theenumi.}
\makeatother
\begin{enumerate}
\item \textbf{SCOP (2018)}, Students Conference on Optics and Photonics, PRL Ahmedabad \textit{\textbf{(Best Poster)}}.
\item  Research Conclave, IIT Ropar \textbf{(2019, 2018)}, \textit{\textbf{(Outstanding Research Award (2019))}}.
\item \textbf{ICOL (2019)}, International Conference on Optics and Electro-optics”,  
IRDE\\ (DRDO), Dehradun.
\item \textbf{ICNIB (2019)}, 5th International Conference on Nanostructuring by Ion Beams , IGCAR , Kalpakkam.


\end{enumerate}


 

{\bf Oral Presentation:}
\begin{enumerate}
\item \textbf{LDMAT(2021)}, Low Dimensional Materials Growth, Optical and Electronic Properties, UM-DAE, Mumbai. 
\end{enumerate}
%{\entry*[Coding\hfill]
	%Java, \smallcaps{PHP}, Python, R, \smallcaps{SQL, XML/XSL}, \LaTeX, \ldots
%\entry*[Databases]
	%My\smallcaps{SQL}, Postgre\smallcaps{SQL}, \smallcaps{HSQL}, \smallcaps{SQL}ite, LotusNotes.
%\entry*[Web Dev]
	%\textsc{Html, css}, JavaScript, Apache Web Server, Tomcat Web Server.
%\entry*[Misc.]
	%Academic research, teaching, training, consultation, \LaTeX\ typesetting and publishing.

